On Learning Latent Models with Multi-Instance Weak Supervision

We consider a weakly supervised learning scenario where the supervision signal is generated by a transition function $\sigma$ of labels associated with multiple input instances. We formulate this problem as \emph{multi-instance Partial Label Learning (multi-instance PLL)}, which is an extension to the standard PLL problem. Our problem is met in different fields, including latent structural learning and neuro-symbolic integration. Despite the existence of many learning techniques, limited theoretical analysis has been dedicated to this problem. In this paper, we provide the first theoretical study of multi-instance PLL with possibly an unknown transition $\sigma$. Our main contributions are as follows. Firstly, we propose a necessary and sufficient condition for the learnability of the problem. This condition non-trivially generalizes and relaxes the existing small ambiguity degree in the PLL literature, since we allow the transition to be deterministic. Secondly, we derive Rademacher-style error bounds based on a top-$k$ surrogate loss that is widely used in the neuro-symbolic literature. Furthermore, we conclude with empirical experiments for learning under unknown transitions. The empirical results align with our theoretical findings; however, they also expose the issue of scalability in the weak supervision literature.

==> sections/experiments.tex <==
\section{Experiments} \label{section:experiments} \todo[]{Merge with conclusions to save space?}

\todo[]{Weighted sum is very expressive as it can model conjunction and disjunction.}
\todo[]{Discuss why other techniques are not applicable.}
Our empirical evaluation aims to validate the results from Section~\ref{section:known-mapping-multi-classifiers} \kaifu{Section 5?}: that we can learn classifiers under unknown transitions. We use an extension of the setting presented in Example~\ref{example:ambiguity}, namely the weighted sum of 2, 4 and 8 digits.  

\textbf{Baselines.} As baselines, we considered multiple state-of-the-art neurosymbolic learning techniques, namely DeepProbLog (DLog) \cite{DBLP:journals/corr/abs-1907-08194}, DeepProbLog with approximate techniques (DLog-GM) \cite{deepproblog-approx}, NeuroLog (NLog) \cite{neurolog}, NeurASP (NASP) \cite{neurasp}, ABL \cite{ABL} and the entropy maximization technique from \cite{iclr2023} denoted as ENT. As these techniques are not designed for structure learning, but for learning classifiers, we employed a simple trick: reducing our setting to learning under known transitions. To establish this reduction, we considered weights in $\{1,2,3,4,5\}$ and used neural classifiers to learn those weights. The inputs to those classifiers are constant signals, e.g., in each iteration, we were providing the weight classifier with the same signal $W_i$ for the $i$-th weight.     
Additionally, we considered standard supervised learning (SL) as a baseline. 

\textbf{Results.} 
\begin{itemize}
\item For $M=2$ training works well-- even better than standard SL.
\item Higher $k$, means better accuracy.
\item This is the key: Scalability is an issue.  
\end{itemize}

\todo[]{Merge Table 2 with 3 to save space.}
\begin{table}[t] 
    \caption{Results on WEIGHTED-SUM for $M=2$. Mean accuracy over 10 different runs. \#0, \#8 and \#16 denote the \# samples used to pretrain the MNIST classifier. All neurosymbolic techniques are trained with \#4K samples. SL is trained with \#4K and \#8K samples, respectively.}
\begin{adjustbox}{max width= \textwidth}
\begin{tabular}{p{0.5cm} p{1.5cm} p{1.5cm} p{1.5cm} p{2.3cm} p{1.5cm} p{2cm} p{1.5cm} p{1.5cm}}
	    & SL (\#4K) & SL (\#8K) & DLog \cite{DBLP:journals/corr/abs-1907-08194} & DLog-A \cite{deepproblog-approx} & NLog \cite{neurolog} & NASP \cite{neurasp} & ABL \cite{ABL} & ENT \cite{iclr2023} \\ \hline
     \#0      & $0.93$   & $0.96$ &  $0.96$    &  R       &   0.97   &  0.21    &  0.09   &  0.40 \\ 
     \#8      & $0.93$   & $0.96$ &  $0.96$    &  R       &   0.97   &  0.21    &  0.10   &  0.43 \\ 
     \#16     & $0.93$   & $0.96$ &  $0.96$    &  R       &   0.97   &  0.21    &  0.11   &  0.49 \\ 
\end{tabular}
\end{adjustbox}
\label{tab:benchmarks}
\end{table}

\begin{table}[t]
    \caption{Results on WEIGHTED-SUM for $M=2$. Mean accuracy over 10 different runs for NeuroLog \cite{neurolog} using \#4K samples. \#8 and \#16 denote the \# samples used to pretrain the MNIST classifier.}
%\begin{adjustbox}{max width= \textwidth}
\begin{tabular}{p{0.5cm} p{1.5cm} p{1.5cm} p{1.5cm} }
	       & top-3  & top-5 & top-$\infty$ \\ \hline
     \#8      &  0.65  & 0.68 & 0.97   \\ 
     \#16     &  0.8  &  0.87 &  0.97  \\ 
\end{tabular}
%\end{adjustbox}
\label{tab:M2-approx}
\end{table}

\begin{table}[t]
        \caption{Results on WEIGHTED-SUM for $M=4$ and $M=8$. 
        Mean accuracy over 10 different runs. \#0, \#8 and \#16 denote the \# samples used to pretrain the MNIST classifier. Both techniques are trained using \#10K samples.}
%\begin{adjustbox}{max width= \textwidth}
\begin{tabular}{p{2.5cm} p{0.8cm} p{0.8cm} p{0.8cm} | p{0.8cm} p{0.8cm} p{0.8cm}}
       & \multicolumn{3}{c}{M=4} & \multicolumn{3}{c}{M=8} \\\hline
       & \#0 & \#8 & \#16 & \#0 & \#8 & \#16 \\ \hline
       DLog-A \cite{deepproblog-approx} &  & 0.20 & 0.26 & N/A & N/A & N/A  \\
       NLog \cite{neurolog} & R & R & 0.32 & R & R & R \\
\end{tabular}
%\end{adjustbox}
\label{tab:M4-M8-approx}
\end{table}


\section{Conclusions} \label{section:conclusions}

In this work, we formulated the problem of multi-instance partial label learning, which extends the classical PLL problem and has significant connections with latent structural learning and neuro-symbolic learning. 
We introduced minimal distributional assumptions that enabled us to establish ERM-learnability and derive error bounds using top-$k$ semantics losses.
Importantly, our assumption exhibits a greater level of flexibility compared to the single-instance problem, as it allows for deterministic transitions. 
This finding suggests the interaction of multiple instances and classifiers in forming the partial labels can potentially facilitate weakly supervised learning.

\textbf{Limitations and future work.}
Although our proposed conditions are minimal and necessary, they can be too restrictive in practical problems.
Nevertheless, the data distributions in real learning scenarios are typically not concentrated or adversarial.
Therefore, for future work, we will assume a certain degree of smoothness for the data distribution to relax the learning conditions.

==> sections/known-mappings.tex <==
\section{Learning with Known Transition} \label{section:ambiguity}

In this section, we study the problem of PLL under the assumption that the transition $\sigma$ is known to the learner.
We start with the case of learning a single classifier and provide a necessary and sufficient condition for learnability (Proposition \ref{ERM-learnability-1-unambiguity}), a sufficient condition for achieving faster convergence (Proposition \ref{ERM-learnability}) as well as an error bound for learning with a top-$k$ surrogate loss (Theorem \ref{thm:pll-error-bound}).
Furthermore, we extend the analysis to the case where we learn multiple classifiers simultaneously.

% ------------------------------------------------------------------
% Learning with single classifier
% ------------------------------------------------------------------


\subsection{Learning with A Single Classifier} \label{section:learning-conditions}

% why not use classical condition
As discussed in Section~\ref{section:related}, learnability for the standard PLL problem \cite{cour2011, learnability-pll} requires that for any input $x$, the maximum probability of that a distractor label co-occurs with the gold one is strictly less than one.
% ; a probability equal to zero reduces to traditional supervised learning. 
However, this assumption is violated in our multi-instance extension of PLL, as demonstrated in Example~\ref{example:motivating}, where three possible combinations of labels \emph{always} exist when the target sum is 2.
Therefore, we need to develop new methods to address this challenge and prove the learnability of our problems.

% To show learnability under the partial zero-one loss (defined in Section~\ref{section:preliminaries}), we need to bound the partial risk ${ \+R^{01}_\:P(f;{\sigma}) }$ by the risk ${ \+R^{01} (f) }$. Assuming that \emph{misclassifying any input $x_i$ results in a different target $s$}, ${ \+R^{01}_\:P(f;{\sigma}) }$ is lower bounded by the probability of misclassifying any of ${x_1, \dots, x_M}$ multiplied by the probability of correctly classifying the remaining ${M-1}$ inputs. We refer to a mapping $\sigma$ for which flipping a label in an input $\_y$ leads to a different target, as \emph{1-unambiguous}:  

% M-unambiguity
\paragraph{A necessary and sufficient condition for learnability.}
To establish the learnability with partially labeled data, we aim to bound the classification risk ${\+R^{01} (f)}$ by the partial risk ${ \+R^{01}_\:P(f;{\sigma})}$. 
In order to achieve this goal, it is necessary for the mapping $\sigma$ to exhibit a certain degree of instability so that classification errors will lead to inconsistencies with the observed partial label.
This idea is formalized by the following definition.

\begin{definition}[$M$-unambiguity] \label{definition:M-unambiguous-mapping}
    Mapping $\sigma$ is \emph{$M$-unambiguous} if  
    for any $\_y \in \+Y^M$ having the same label $l$ in all positions, 
    the vector $\_y'$ that results after flipping each occurrence of $l$ to $l' \neq l$ satisfies ${\sigma(\_y') \neq \sigma(\_y)}$. 
\end{definition}

We show $M$-unambiguity is necessary and sufficient to guarantee the consistency of PLL.

\begin{restatable}[ERM learnability under $M$-unambiguity]{proposition}{ermlearnability} \label{ERM-learnability-1-unambiguity}
    If $\sigma$ is $M$-unambigous,
    then for any classifier $f$, we have that:
    \begin{equation}
    \label{eqn:M-unambiguity-upper-bound}
    \begin{aligned}
        \+R^{01}(f)
        \le O(\+R^{01}_\:P(f;\sigma)^{1/M})
    \end{aligned}
    \end{equation}
    Moreover, if $\sigma$ is not $M$-unambiguous, then learning from partial labels is arbitrarily difficult, in the sense that a classifier $f$ with perfect partial risk ${\+R^{01}_\:P(f;\sigma)=0}$ can have a risk of ${\+R^{01}(f)=1}$.
\end{restatable}

\paragraph{Achieving a faster rate.}
The above $M$-unambiguity makes minimal assumptions for the transition $\sigma$ by only constraining the diagonal cases.
Consequently, the convergence rate presented in \eqref{eqn:M-unambiguity-upper-bound} becomes slower as $M$ increases.
To achieve a faster convergence rate, we propose the following condition, which states that the mapping $\sigma$ is sensitive to 1-bit perturbations.

\begin{definition}[1-unambiguity] \label{definition:1-unambiguous-mapping}
    The mapping $\sigma$ is \emph{1-unambiguous} if there exists an index 
    ${1 \leq i \leq M}$, such that flipping the $i$-th label of any ${\_y \in \+Y^M}$, results in a vector $\_y'$ with ${\sigma(\_y') \neq \sigma(\_y)}$.
\end{definition}

Now we show if $\sigma$ is both 1- and $M$-unambiguous, then the classification risk can be bounded linearly by the partial risk.

% Below, we demonstrate an example of 1-unambiguity. 
% \begin{example}
%     The mapping $\sigma$ from Example~\ref{example:motivating} that maps two digits to their sum is 1-unambiguous.   
%     For instance, if the gold labels for an input ${(x_1, x_2)}$ are $(0,9)$-- implying a target sum equal to nine-- and $f$ misclassifies $x_1$ to 0, then the original target is violated as 1+9=10.
% \end{example}

% While the mapping that describes a two-digit addition is 1-unambiguous, we can find mappings that violate this assumption, as demonstrated below:

% \begin{example} \label{example:M-unambiguous-mapping}
%     Consider a variant of Example~\ref{example:motivating}, where instead of taking the sum, we take the product of two digits, inducing a mapping ${\sigma^*(y_1,y_2) = y_1 \times y_2}$. Mapping $\sigma^*$ is not 1-unambiguous. For instance, consider the vector of labels $\_y = (0,1)$. The vector $\_y' = (0,2)$ that results after flipping the second label to 2, leads also to product 0, violating the condition that ${\sigma(\_y) \neq \sigma(\_y')}$. 
% \end{example}

% Nevertheless, for mappings that are not 1-unambiguous, we can still bound ${\+R^{01}_\:P(f;{\sigma}) }$ by ${ \+R^{01} (f) }$. This can happen when simultaneously flipping all $M$ labels for any input $\_y$ of the form ${(l,\dots,l)}$ will result in a vector $\_y'$ of the form ${(l',\dots,l')}$ with ${\sigma^*(\_y') \neq \sigma^*(\_y) }$. Hence, ${\+R^{01}_\:P(f; {\sigma}) }$ is lower bounded by the probability that $f$ misclassifies each $x_i$, for ${1 \leq i \leq M}$, to $l'$ instead of $l$. The mapping $\sigma^*$ from Example~\ref{example:M-unambiguous-mapping} satisfies this property. 
% Below, we present $M$-unambiguity to capture $M$ simultaneous label flips: 

%Similarly to 1-unambiguity, $M$-unambiguity also provides a lower bound for the partial risk ${\+R_\:P(\_f;\ell^{01}_{\sigma}) }$. The lower bound in that case is the probability of misclassifying all the ${x_1, \dots, x_M}$ as of label $l'$ instead of $l$.

\begin{restatable}[ERM learnability under unambiguity]{proposition}{ermlearnability} \label{ERM-learnability}
    If $\sigma$ is both 1- and $M$-unambigous,
    then for any classifier $f$, we have that:
    \begin{equation}
    \begin{aligned}
        \+R^{01}(f)
        \le O(\+R^{01}_\:P(f;\sigma))
    \end{aligned}
    \end{equation}
\end{restatable}

In the following, we provide examples of partial labels that satisfy or not our proposed conditions.

\begin{example}[Examples of (un)ambiguous mappings]\leavevmode
   \begin{enumerate}[leftmargin=*]
       \item ($M$-sum) Let $\+Y = \{0,1,\dots, 9\}$ and $\sigma(y_1,\dots,y_M) = \sum_{i=1}^M y_i$. Then $\sigma$ is both 1-unambiguous and $M$-unambiguous.
       
       \item ($M$-product) Let $\+Y = \{0,1,\dots, 9\}$ and $\sigma(y_1, \dots, y_M) = \prod_{i=1}^M y_i$ be the product of the input digits. Then $\sigma$ is $M$-unambiguous but not $1$-unambiguous since (1) $y^{M-1} \times 0 \equiv 0$ and (2) $y^M \ne (y')^M$ for any $y \ne y'$.
       
       \item (Exclusive Or) Let $\+Y = \{0,1\}$ and $\sigma(y_1,y_2) = \-1\{y_1 \ne y_2\}$. Then $\sigma$ is ambiguous since $\sigma(1,1) = \sigma(0,0)$.
   \end{enumerate}
\end{example}

\paragraph{Intermediate rates.} 
Furthermore, we provide the following example to show that the convergence rate can be $\+R^{01}(f) \le O((\+R^{01}_\:P(f;\sigma))^{1/I})$ for any $I \in [M]$. To give a sufficient condition for achieving these intermediate rates, in the appendix, we introduce the notion of $I$-unambiguit that generalizes the concept of $1$-unambiguity.

\begin{example}[Slower rates can be achieved]
\kaifu{TODO, should not be difficult.}
%     Let $M=2$, $\+Y = \{0,1\}$ and $\sigma(y_1,y_2) = y_1 \times y_2$. Suppose the distribution is concentrated on an instance with label $0$. Then, $s$ is misclassified iff both labels are misclassified. Therefore, ${\+R^{01}_\:P(f;{\sigma}) = (\+R^{01}(f))^2}$, resulting in a convergence rate of order $1/2$.
\end{example}

%\todo[]{Clean and add Kaifu's examples.}
%\begin{example}[Examples of (un)ambiguous mappings]\leavevmode
%    \begin{enumerate}
%        \item (sum) Let $\+Y = \{0,1,\dots, 9\}$ and $\sigma(y_1,\dots,y_M) = \sum_{i=1}^M y_i$. Then $\sigma$ is I-unambiguous for any $I \in [M]$ since $Iy + y_{I+1} \dots + y_{M} \ne Iy' + y_{I+1} \dots + y_{M}$ for any $y\ne y'$.
%        
%        \item (product) Let $\+Y = \{0,1,\dots, 9\}$ and $\sigma(y_1, \dots, y_M) = \prod_{i=1}^M y_i$ be the product of the input digits. Then $\sigma$ is $M$-unambiguous but not $M'$-unambiguous for any $M' < M$ since (1) $y^{M-1} \times 0 \equiv 0$ and (2) $y^M \ne (y')^M$ for any $y \ne y'$.
%        
%        \item (exclusive or) Let $\+Y = \{0,1\}$ and $\sigma(y_1,y_2) = \-1\{y_1 \ne y_2\}$. Then $\sigma$ is ambiguous since $\sigma(1,1) = \sigma(0,0)$.
%    \end{enumerate}
%\end{example}

% ------------------------------------------------------------------
% Top-k approximation
% ------------------------------------------------------------------

\subsection{Top-$k$ Approximation} \label{section:ambiguity:top-k}
\todo[]{Kaifu said that the special case $k=1$ coincides with the infimum loss \cite{structured-prediction-pll} and minimal loss \cite{progressive-pll} in the PLL literature. Is that still true?}

Section~\ref{section:learning-conditions} discusses learnability under the zero-one loss. It is known that ERM for classification problems under that loss is intractable even for linear classifiers \cite{intractability-of-01-loss}. However, in our case, there is a second source of intractability: that of enumerating the entries of $\sigma$. For instance, in Example~\ref{example:motivating}, we have to enumerate all  $10 \times 10$ digit combinations to populate $\sigma$. However, that might be impractical, or even infeasible for more complex mappings as demonstrated in \cite{scallop,neurolog}. Recall that the only reason for which we consider all possible combinations of labels that would lead us to the desired target is because we \emph{don’t know the gold annotation}: if we knew the gold annotation, we would simply consider that one. 

A popular approximation is the top-$k$ one, according to which, we consider only the most likely label combinations, where the probability ${P_{f(\_x)}(\_y)}$ of a label combination $\yp$ assuming we are given a training instance $(\xp,s)$ and classifier $f$ is defined by
${P_{f(\_x)}(\_y) \defeq \prod^M_{i=1} f^{y_i}(x_i)}$.
Returning back to Example~\ref{example:motivating}, instead of considering 
all three combinations $(2,0)$, $(1,1)$ and $(0,2)$ assuming a target $s=2$, we can consider only the 
first and the last combination, if the probabilities of the first and the second image being 1 are way lower than those of being 0 or 2.  
This approximation is quite intuitive in cases where $f$ has been pre-trained. 
However, it also works in scenarios where no pre-training takes place \cite{scallop}. 
%The intuition behind this loss comes from the probabilistic logic programming community \cite{DBLP:journals/corr/abs-1907-08194,scallop}, where, given ${\_x}$, we aim to maximize the probability of deriving $s$, denoted by ${P_{f(\_x)}(s)}$. Assuming that ${\_y_1, \dots, \_y_N}$ are all the tuples of labels so that ${\sigma(\_y_i)=s}$, we have
%\begin{align}
%	P_{f(\_x)}(s) \leq 1 - \prod^N_{i=1} (1 - P_{f(\_x)}(\_y_i))
%\end{align} 
%where equality holds only when the $\_y_i$’s share no labels. 
We are now ready to define the top-$k$ \textit{partial loss}. 
\todo[]{Need to check if the learnability proof works; if not, then easy change is to take the product of the probabilities as the loss.}

\begin{definition}[Top-$k$ loss] 
\label{definition:top-k-loss}
The \emph{top-$k$ loss}, ${k \ge 1}$, subject to classifier $f$, $s \in \Sp$ and $\sigma$ is   
    \begin{equation}
        \begin{aligned}
            \ell^{k}_{\sigma}(f(\_x), s)
            \defeq -\log \left( 1 - \prod^k_{i=1} (1 - P_{f(\_x)}(\_y^{(i)})) \right) \label{equation:top-k-loss}
        \end{aligned}
    \end{equation}
    where ${\_y^{(1)}, \dots, \_y^{(k)}}$ are the tuples of labels with the $k$ highest probabilities and
    ${\sigma(\_y^{(i)}) = s}$, for each ${1 \leq i \leq k}$.
\end{definition}
%Notice that, differently from the partial zero-one loss, we omit $\sigma$, since it does not play a role.
%The logarithmic term in the right-hand side of \eqref{equation:top-k-loss} might look cryptic at a first glance. However, it has its origins in the probabilistic logic programming community \cite{pmlr-v80-xu18h,DBLP:journals/corr/abs-1907-08194,scallop}: it is an upper bound to the probability of either of ${\_y^{(1)}, \dots, \_y^{(k)}}$ being the gold labels for $\_x$. In fact, it is a lower bound to the semantic loss \cite{pmlr-v80-xu18h}\todo[]{Check correctness of the statement.}. 


The \emph{top-$k$ partial classification risk} subject to 
$\sigma$ is given by 
\begin{align}
    \+R^{k}_\:P(f;{\sigma}) \defeq \-E_{(X_1,\dots,X_M,S) \sim \+D_\:P}[\ell^{k}_{\sigma}(f(X_1,\dots,X_M),S)]            \label{eq:partial-top-k-risk-single-classifier}
\end{align}

\begin{restatable}[Consistency of the top-$k$ partial loss]{proposition}{topkconsistency}
    \label{topkconsistency}
    For any $k \ge 1$ and any classifier $f$, we have: 
    \begin{equation}
    \label{eq:top-k-loss-as-upper-bound}
    \begin{aligned}
        \+R^{01}_\:P(f;{\sigma}) 
        \le \log\left(\frac{k+1}{k}\right) \+R^k_\:P(f;{\sigma}) 
    \end{aligned}
    \end{equation}
\end{restatable}

% ------------------------------------------------------------------
% Error bound
% ------------------------------------------------------------------

\subsection{Error Bound for multi-instance PLL} \label{section:ambiguity:error-bound}

We upper bound the classification risk with the empirical top-$k$ partial risk from Definition \ref{definition:top-k-loss}.

\begin{restatable}[Error bound under unambiguity]{theorem}{rademacherpll} 
    \label{thm:pll-error-bound}
    For a mapping $\sigma$ that is both $1$- and $M$-unambigous and any classifier $f$, we have with probability $1-\delta$, for $\delta \in (0,1)$:
    \begin{equation}
    \begin{aligned}
        \+R^{01}(f)
        \le (1 + c(c-1))^{M-1}(k+1) \left(
            \hat{\+R}^k_{\:P}(f;{\sigma};\+T_{\:P})
            + 2M\mathfrak{R}_{m_\:P} (\+F)
            + \sqrt{\frac{\log(1/\delta)}{2m_\:P}}
        \right)
    \end{aligned}
    \end{equation}
    where $\hat{\+R}^k_{\:P}(f;{\sigma};\+T_{\:P})$ is the empirical counterpart of \eqref{eq:partial-top-k-risk-single-classifier}.
\end{restatable}

% ------------------------------------------------------------------
% Learning with Multiple Classifiers
% ------------------------------------------------------------------

\subsection{Learning with Multiple Classifiers} \label{section:multi-classifier}

\begin{definition}[Strong-unambiguity]
    Mapping $\sigma$ is \emph{strongly-unambiguous} if for any
    $i \in [M]$, flipping the $i$-th label of any ${\_y \in \+Y^{M}}$, results in a vector $\_y'$ with ${\sigma(\_y') \neq \sigma(\_y)}$.
\end{definition} \todo[]{Careful with the notation. I use $L$ to denote the number of different classifiers. You use $M$. $M$ above is the dimension of the input vector in the single classifier case. I modified the definition to comply with my notation.}

\begin{restatable}[ERM learnability under strong-unambiguity]{proposition}{ermlearnabilitymulticlassifier}
    \label{ERM-learnability-multiclassifier}
    If a mapping $\sigma$ is strongly-unambiguous and there is a constant $R < 1$ \todo[]{Incosistency with the definition for a single classifier. Perhaps, we can do the same? Now it reads strange.} such that $\+R^{01}(f) \le R$ for all $f \in \+F$, then for any classifier $\_f$,
    \begin{equation}
    \begin{aligned}
        \+R^{01}(\_f)
        \le \frac{\+R^{01}_\:P(\_f; {\sigma})}{(1-R)^{M-1}}
    \end{aligned}
    \end{equation}
    Moreover, if $\sigma$ is not strongly-unambiguous, then learning from partial labels is arbitrarily difficult, in the sense that a classifier $\_f$ with perfect partial risk ${\+R^{01}_\:P(\_f; {\sigma})=0}$ can have a risk of ${\+R^{01}(\_f)=1}$.
\end{restatable}

\begin{definition}[Top-$k$ loss for multiple classifiers] \todo[]{Problematic notation}
    For ${k \ge 1}$, the \emph{top-$k$ partial loss} subject to scoring function $\_f$ and $s \in \Sp$ is given by   
    \begin{equation}
        \begin{aligned}
            \ell^{k}_{\sigma}(\_f(\_x),s)
            \defeq -\log \left( 1 - \prod^k_{i=1} (1 - P_{\_f(\_x)}(\_y^{(i)})) \right)
        \end{aligned}
    \end{equation}
    where ${\_y^{(1)}, \dots, \_y^{(k)}}$ are defined as above.
\end{definition}

